Towards Reconstructing and Recognizing Objects behind Fragmented Occlusion using Video

Perceiving objects through fragmented occlusions, such as foliage, is a natural capability of the human visual system but remains a fundamental challenge for computer vision. This work addresses the problem of object reconstruction, or de-occlusion, in the presence of high-density, fragmented occlusions. We propose a reconstruction framework that operates on a sequence of grayscale images of a moving object, acquired by a single camera, either stationary or in motion. The algorithm estimates the object's relative positions across frames by jointly registering the images and optimizing the alignment parameters to maximize the contrast of their average, referred to as the integrated image. This integrated image serves as the reconstructed representation of the object. Experimental evaluations on both synthetic and real video sequences demonstrate the feasibility of accurate reconstruction under occlusion densities exceeding 90%. The proposed approach is competitive with synthetic aperture techniques, which are limited to static objects and require complex camera setup with careful calibration. Furthermore, we show that the integrated image enables reliable object classification under severe occlusion when used as input to standard, off-the-shelf classifiers.

==> fig/method/method.tex <==
\begin{figure}
\centering
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,239); %set diagram left start at 0, and has height of 239
%Image [id:dp9823312449412047] 
\draw (65,60) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000004.png}};
%Shape: Square [id:dp37823830672662806] 
\draw   (30,25) -- (100,25) -- (100,95) -- (30,95) -- cycle ;
%Image [id:dp4758062605889479] 
\draw (190,198) node  {\includegraphics[width=52.5pt,height=52.5pt]{018-193-synex-s_7_0_-n_43_-msi-u_-06_00_-v_-04_00_.png}};
%Image [id:dp24743081741386708] 
\draw (115,198) node  {\includegraphics[width=52.5pt,height=52.5pt]{191-193-synex-s_7_0_-n_43_-msi-u_+05_00_-v_+04_00_.png}};
%Image [id:dp8876692678872601] 
\draw (40,198) node  {\includegraphics[width=52.5pt,height=52.5pt]{009-193-synex-s_7_0_-n_43_-msi-u_-07_00_-v_+02_00_.png}};
%Image [id:dp24930275116578715] 
\draw (245,60) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000007.png}};
%Shape: Square [id:dp023320660730997478] 
\draw   (210,25) -- (280,25) -- (280,95) -- (210,95) -- cycle ;
%Right Arrow [id:dp38848073154789287] 
\draw   (27.5,120) -- (27.5,133.5) -- (30,133.5) -- (25,140) -- (20,133.5) -- (22.5,133.5) -- (22.5,120) -- cycle ;
%Straight Lines [id:da8328753277395858] 
\draw    (5,154) -- (308,154) ;
\draw [shift={(310,154)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Curve Lines [id:da2613568912233376] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (95,154) .. controls (141.6,105.13) and (156,109.53) .. (190,154) ;
%Straight Lines [id:da6073969193373644] 
\draw [line width=0.75]  [dash pattern={on 0.84pt off 2.51pt}]  (145,118) -- (145,153) ;
%Straight Lines [id:da04842042669159696] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (120,118) -- (170,118) ;
%Right Arrow [id:dp4443667358488773] 
\draw   (230,195.5) -- (243.5,195.5) -- (243.5,193) -- (250,198) -- (243.5,203) -- (243.5,200.5) -- (230,200.5) -- cycle ;
%Image [id:dp10804598175718172] 
\draw (170,60) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000013.png}};
%Shape: Square [id:dp10867820487776847] 
\draw   (135,25) -- (205,25) -- (205,95) -- (135,95) -- cycle ;

%Image [id:dp6091230210785437] 
\draw (160,60) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000013.png}};
%Shape: Square [id:dp3576154300419002] 
\draw   (125,25) -- (195,25) -- (195,95) -- (125,95) -- cycle ;

%Image [id:dp8063807686368601] 
\draw (150,60) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000013.png}};
%Shape: Square [id:dp2033991801118069] 
\draw   (115,25) -- (185,25) -- (185,95) -- (115,95) -- cycle ;

%Image [id:dp22677518491616722] 
\draw (140,60) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000013.png}};
%Shape: Square [id:dp4431813774395291] 
\draw   (105,25) -- (175,25) -- (175,95) -- (105,95) -- cycle ;

%Image [id:dp03349328429158771] 
\draw (60,65) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000004.png}};
%Shape: Square [id:dp49069676680903274] 
\draw   (25,30) -- (95,30) -- (95,100) -- (25,100) -- cycle ;

%Image [id:dp48274994116639247] 
\draw (55,70) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000004.png}};
%Shape: Square [id:dp9673269365421004] 
\draw   (20,35) -- (90,35) -- (90,105) -- (20,105) -- cycle ;

%Image [id:dp3245050001813812] 
\draw (50,75) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000004.png}};
%Shape: Square [id:dp6800036061547704] 
\draw   (15,40) -- (85,40) -- (85,110) -- (15,110) -- cycle ;

%Image [id:dp27968784461675] 
\draw (255,65) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000007.png}};
%Shape: Square [id:dp6339524869360224] 
\draw   (220,30) -- (290,30) -- (290,100) -- (220,100) -- cycle ;

%Image [id:dp34123087170754884] 
\draw (265,70) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000007.png}};
%Shape: Square [id:dp2791660211141528] 
\draw   (230,35) -- (300,35) -- (300,105) -- (230,105) -- cycle ;

%Image [id:dp41696824494309903] 
\draw (275,75) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000007.png}};
%Shape: Square [id:dp49812930542111467] 
\draw   (240,40) -- (310,40) -- (310,110) -- (240,110) -- cycle ;


% Text Node
\draw (57,2.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\mathcal{F}_{i}$};
% Text Node
\draw (141,2.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\mathcal{F}_{j}$};
% Text Node
\draw (65,130.5) node  [font=\footnotesize] [align=left] {Image\\Integration};
% Text Node
\draw (128,137) node  [font=\small,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$f$};
% Text Node
\draw (193,146) node  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$\mathbf{\theta }^{*} =\ \text{vec}\left(\mathcal{F}^{*}\right)$};
% Text Node
\draw (250.5,2.4) node [anchor=north] [inner sep=0.75pt]  [font=\small]  {$\mathcal{F}^{*}$};
% Text Node
\draw (286,158.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\mathbf{\theta }$};
% Text Node
\draw (195,116.5) node  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$\frac{\partial f}{\partial \mathbf{\theta }} =0$};
% Text Node
\draw (268.5,220.5) node  [font=\footnotesize] [align=left] {{\small Image Contrast}};
% Text Node
\draw (271.5,196.5) node  [font=\small,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$f( \ \ \ \ )$};
% Text Node
\draw (115,62) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{59.39pt}\setlength\topsep{0pt}
\begin{center}
\textbf{Motion}\\\textbf{Compensation}
\end{center}

\end{minipage}};
% Text Node
\draw (274.5,196.5) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$\mathcal{F}$};
% Text Node
\draw (232,160.4) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$\hat{I}_{r}$};
\end{tikzpicture}
%\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
%\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%%uncomment if require: \path (0,231); %set diagram left start at 0, and has height of 231
%%Image [id:dp8394074508878957] 
%\draw (165,57) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000015.png}};
%%Image [id:dp6921969676138064] 
%\draw (155,57) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000007.png}};
%%Image [id:dp7612129644433351] 
%\draw (145,57) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000004.png}};
%%Image [id:dp06148347941239918] 
%\draw (135,57) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000001.png}};
%%Image [id:dp4922618125639686] 
%\draw (55,57) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000015.png}};
%%Image [id:dp48475042486910425] 
%\draw (50,62) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000007.png}};
%%Image [id:dp25253804473203634] 
%\draw (45,67) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000004.png}};
%%Image [id:dp5559227129944693] 
%\draw (40,72) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000001.png}};
%%Image [id:dp4758062605889479] 
%\draw (190,190) node  {\includegraphics[width=52.5pt,height=52.5pt]{152-man-msi-u(-03.00)-v(-05.00).png}};
%%Image [id:dp24743081741386708] 
%\draw (115,190) node  {\includegraphics[width=52.5pt,height=52.5pt]{133-man-msi-u(-04.00)-v(-03.00).png}};
%%Image [id:dp8876692678872601] 
%\draw (40,190) node  {\includegraphics[width=52.5pt,height=52.5pt]{040-man-msi-u(-09.00)-v(+09.00).png}};
%%Image [id:dp0990335884697261] 
%\draw (275,87) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000015.png}};
%%Image [id:dp7480154043898022] 
%\draw (265,77) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000007.png}};
%%Image [id:dp7018494237596427] 
%\draw (255,67) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000004.png}};
%%Image [id:dp01815355813087982] 
%\draw (245,57) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000001.png}};
%%Right Arrow [id:dp38848073154789287] 
%\draw   (17.5,115) -- (17.5,128.5) -- (20,128.5) -- (15,135) -- (10,128.5) -- (12.5,128.5) -- (12.5,115) -- cycle ;
%%Straight Lines [id:da8328753277395858] 
%\draw    (5,146) -- (308,146) ;
%\draw [shift={(310,146)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%%Curve Lines [id:da2613568912233376] 
%\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (95,146) .. controls (141.6,97.13) and (156,101.53) .. (190,146) ;
%%Straight Lines [id:da6073969193373644] 
%\draw [line width=0.75]  [dash pattern={on 0.84pt off 2.51pt}]  (145,110) -- (145,145) ;
%%Straight Lines [id:da04842042669159696] 
%\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (120,110) -- (170,110) ;
%%Right Arrow [id:dp4443667358488773] 
%\draw   (230,187.5) -- (243.5,187.5) -- (243.5,185) -- (250,190) -- (243.5,195) -- (243.5,192.5) -- (230,192.5) -- cycle ;
%% Text Node
%\draw (46,3.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\mathcal{F}_{i}$};
%% Text Node
%\draw (141,3.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\mathcal{F}_{j}$};
%% Text Node
%\draw (55,124.5) node  [font=\footnotesize] [align=left] {Image\\Integration};
%% Text Node
%\draw (128,129) node  [font=\small,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$f$};
%% Text Node
%\draw (193,138) node  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$\mathbf{\theta }^{*} =\ \text{vec}\left(\mathcal{F}^{*}\right)$};
%% Text Node
%\draw (250.5,4.4) node [anchor=north] [inner sep=0.75pt]  [font=\small]  {$\mathcal{F}^{*}$};
%% Text Node
%\draw (286,150.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\mathbf{\theta }$};
%% Text Node
%\draw (195,108.5) node  [font=\small,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$\frac{\partial f}{\partial \mathbf{\theta }} =0$};
%% Text Node
%\draw (268.5,212.5) node  [font=\footnotesize] [align=left] {{\small Image Contrast}};
%% Text Node
%\draw (271.5,188.5) node  [font=\small,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$f( \ \ \ \ )$};
%% Text Node
%\draw (110,41) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 255; green, 255; blue, 255 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{59.39pt}\setlength\topsep{0pt}
%\begin{center}
%\textbf{Motion}\\\textbf{Compensation}
%\end{center}
%\end{minipage}};
%% Text Node
%\draw (274.5,188.5) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$\mathcal{F}$};
%% Text Node
%\draw (232,152.4) node [anchor=north west][inner sep=0.75pt]  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$\hat{I}_{r}$};
%\end{tikzpicture}
\caption{Stack $\mathcal{J}$ of motion compensated images (top) is combined into the integrated image (bottom). The algorithm then estimates the contrast of $\hat{I}_r$ for different motions, $\mathcal{F}_i$, $\mathcal{F}_j$ and $\mathcal{F}^*$. The correct motion $\vec{\theta^*}$ and the reconstruction of the occluded object is simultaneously found with $\hat{I}_r$ at its maximal contrast.}
\label{fig:method}
\end{figure}


==> fig/method/reconstruction.tex <==
\begin{figure}
\centering
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,191); %set diagram left start at 0, and has height of 191
%Image [id:dp3586536575166229] 
\draw (260,135) node  {\includegraphics[width=52.5pt,height=52.5pt]{018-193-synex-s_7_0_-n_43_-msi-u_-06_00_-v_-04_00_.png}};
%Image [id:dp8476755818407172] 
\draw (65,120) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000013.png}};
%Image [id:dp528521128664939] 
\draw (35,150) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000001.png}};
%Image [id:dp32039484247245154] 
\draw (185,40) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000007.png}};
%Shape: Cube [id:dp27537841219927306] 
\draw   (0,115) -- (30,85) -- (100,85) -- (100,155) -- (70,185) -- (0,185) -- cycle ; \draw   (100,85) -- (70,115) -- (0,115) ; \draw   (70,115) -- (70,185) ;
%Straight Lines [id:da18563091824141686] 
\draw    (0,80) -- (293,80) ;
\draw [shift={(295,80)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Right Arrow [id:dp2508071575822922] 
\draw   (105,122.5) -- (174,122.5) -- (174,110) -- (220,135) -- (174,160) -- (174,147.5) -- (105,147.5) -- cycle ;
%Image [id:dp8612477166651746] 
\draw (35,40) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000001.png}};
%Image [id:dp234555206537989] 
\draw (260,40) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000013.png}};
%Image [id:dp859638295776253] 
\draw (110,40) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000004.png}};
%Shape: Rectangle [id:dp19442792287953026] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]  (225,100) -- (295,100) -- (295,170) -- (225,170) -- cycle ;
%Shape: Rectangle [id:dp5728586037916805] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]  (150,5) -- (220,5) -- (220,75) -- (150,75) -- cycle ;
% Text Node
\draw (156.5,135) node  [font=\footnotesize] [align=left] {2D Reconstruction};
\end{tikzpicture}
%\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
%\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%%uncomment if require: \path (0,191); %set diagram left start at 0, and has height of 191
%%Image [id:dp47104290043837416] 
%\draw (260,135) node  {\includegraphics[width=52.5pt,height=52.5pt]{152-man-msi-u(-03.00)-v(-05.00)}};
%%Image [id:dp7405952018454847] 
%\draw (65,120) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000015.png}};
%%Image [id:dp915234635332533] 
%\draw (35,150) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000001.png}};
%%Image [id:dp9672841467289804] 
%\draw (185,40) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000007.png}};
%%Shape: Cube [id:dp4205406705364705] 
%\draw   (0,115) -- (30,85) -- (100,85) -- (100,155) -- (70,185) -- (0,185) -- cycle ; \draw   (100,85) -- (70,115) -- (0,115) ; \draw   (70,115) -- (70,185) ;
%%Straight Lines [id:da00141436129154493] 
%\draw    (0,80) -- (293,80) ;
%\draw [shift={(295,80)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%%Right Arrow [id:dp6531249259934829] 
%\draw   (105,122.5) -- (174,122.5) -- (174,110) -- (220,135) -- (174,160) -- (174,147.5) -- (105,147.5) -- cycle ;
%%Image [id:dp47174779799398703] 
%\draw (35,40) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000001.png}};
%%Image [id:dp621632202617581] 
%\draw (260,40) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000015.png}};
%%Image [id:dp2032755680184931] 
%\draw (110,40) node  {\includegraphics[width=52.5pt,height=52.5pt]{0000000004.png}};
%%Shape: Rectangle [id:dp8120879125453699] 
%\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]  (225,100) -- (295,100) -- (295,170) -- (225,170) -- cycle ;
%%Shape: Rectangle [id:dp4020350048772857] 
%\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=1.5]  (150,5) -- (220,5) -- (220,75) -- (150,75) -- cycle ;
%% Text Node
%\draw (156.5,135) node  [font=\footnotesize] [align=left] {2D Reconstruction};
%\end{tikzpicture}
\caption{Reconstructing or de-occluding an object’s shape and appearance from a sequence of occluded images creates an integrated, non-occluded image of the moving object for some reference in the sequence (see the red framed image).}
\label{fig:reconstruction}
\end{figure}
